Optically Selected Compact Stellar Regions and Tidal Dwarf Galaxies in (Ultra)-Luminous Infrared Galaxies

This thesis work is devoted to the analysis of compact star forming regions (knots) in a representative sample of 32 (U)LIRGs. The project is based mainly on optical high angular resolution images taken with the ACS and WFPC2 cameras on board the HST telescope, data from a high spatial resolution simulation of a major galaxy encounter, and with the combination of optical integral field spectroscopy (IFS) taken with the INTEGRAL (WHT) and VIMOS (VLT) instruments. A few thousand knots -a factor of more than one order of magnitude higher than in previous studies- are identified and their photometric properties are characterized as a function of the infrared luminosity of the system and of the interaction phase. These properties are compared with those of compact objects identified in simulations of galaxy encounters. Finally, and with the additional use of IFS data, we search for suitable candidates to tidal dwarf galaxies, setting up constraints on the formation of these objects for the (U)LIRG class. Knots in (U)LIRGs are likely to contain sub-strucutre. Evidence is found that in ULIRGs they are intrinsically more luminous than in less luminous interacting systems due to size-of-sample effects. Furthermore, their sizes and masses are similar to stellar complexes or clumps detected in galaxies at z > 1, unlike local stellar complexes. The star formation in (U)LIRGs is charaterized by a luminosity function with a slope consistent with \alpha = 2, independent of the luminosity of the system. However, it may flatten slightly due to, as simulations suggest, higher knot formation rates at early phases of the interaction. Candidates to tidal dwarf galaxies are identified in the sample. With a production rate of 0.1 candidates per (U)LIRG system, only a few fraction (< 10%) of the general dwarf satellite population could be of tidal origin.

==> autobib.tex <==
\bibitem[Aarseth(1963)]{Aarseth1963}\linkup{autobib:Aarseth1963} Aarseth, S.~J.\ 1963, \mnras, 126, 223\linkads{http://adsabs.harvard.edu/abs/1963MNRAS.126..223A}
\bibitem[Aarseth(1999)]{Aarseth1999}\linkup{autobib:Aarseth1999} Aarseth, S.~J.\ 1999, \pasp, 111, 1333\linkads{http://adsabs.harvard.edu/abs/1999PASP..111.1333A}
\bibitem[Anders et al.(2007)]{Anders2007}\linkup{autobib:Anders2007} Anders, P., Bissantz, N., Boysen, L., de Grijs, R., \& Fritze-v.~Alvensleben, U.\ 2007, \mnras, 377, 91\linkads{http://adsabs.harvard.edu/abs/2007MNRAS.377...91A}
\bibitem[Anderson(1992)]{Anderson1992}\linkup{autobib:Andersson1992} Anderson, C.\ 1992, SIAM Journal on Scientific and Statistical Computing, 13, 923
\bibitem[Athanassoula et al.(1998)]{Athanassoula1998}\linkup{autobib:Athanassoula1998} Athanassoula, E., Bosma, A., Lambert, J.-C., \& Makino, J.\ 1998, \mnras, 293, 369\linkads{http://adsabs.harvard.edu/abs/1998MNRAS.293..369A}
\bibitem[Baldi et al.(2006)]{Baldi2006}\linkup{autobib:Baldi2006} Baldi, A., Raymond, J.~C., Fabbiano, G., Zezas, A., Rots, A.~H., Schweizer, F., King, A.~R., \& Ponman, T.~J.\ 2006, \apj, 636, 158\linkads{http://adsabs.harvard.edu/abs/2006ApJ...636..158B}
\bibitem[Barnes \& Hut(1986)]{Barnes1986}\linkup{autobib:Barnes1986} Barnes, J., \& Hut, P.\ 1986, \nat, 324, 446\linkads{http://adsabs.harvard.edu/abs/1986Natur.324..446B}
\bibitem[Barnes(1988)]{Barnes1988a}\linkup{autobib:Barnes1988a} Barnes, J.~E.\ 1988, \apj, 331, 699\linkads{http://adsabs.harvard.edu/abs/1988ApJ...331..699B}
\bibitem[Barnes et al.(1988)]{Barnes1988b}\linkup{autobib:Barnes1988b} Barnes, J., Hernquist, L.~E., Hut, P., \& Teuben, P.\ 1988, \baas, 20, 706\linkads{http://adsabs.harvard.edu/abs/1988BAAS...20..706B}
\bibitem[Barnes(2004)]{Barnes2004}\linkup{autobib:Barnes2004} Barnes, J.~E.\ 2004, \mnras, 350, 798\linkads{http://adsabs.harvard.edu/abs/2004MNRAS.350..798B}
\bibitem[Barnes \& Hibbard(2009)]{Barnes2009}\linkup{autobib:Barnes2009} Barnes, J.~E., \& Hibbard, J.~E.\ 2009, \aj, 137, 3071\linkads{http://adsabs.harvard.edu/abs/2009AJ....137.3071B}
\bibitem[Bastian et al.(2009)]{Bastian2009}\linkup{autobib:Bastian2009} Bastian, N., Trancho, G., Konstantopoulos, I.~S., \& Miller, B.~W.\ 2009, \apj, 701, 607\linkads{http://adsabs.harvard.edu/abs/2009ApJ...701..607B}
\bibitem[Bate, Bonnell, \& Bromm(2003)]{Bate2003}\linkup{autobib:Bate2003} Bate, M.~R., Bonnell, I.~A., \& Bromm, V.\ 2003, \mnras, 339, 577\linkads{http://adsabs.harvard.edu/abs/2003MNRAS.339..577B}
\bibitem[Baumgardt \& Makino(2003)]{Baumgardt2003}\linkup{autobib:Baumgardt2003} Baumgardt, H., \& Makino, J.\ 2003, \mnras, 340, 227\linkads{http://adsabs.harvard.edu/abs/2003MNRAS.340..227B}
\bibitem[Baumgardt \& Kroupa(2007)]{Baumgardt2007}\linkup{autobib:Baumgardt2007} Baumgardt, H., \& Kroupa, P.\ 2007, \mnras, 380, 1589\linkads{http://adsabs.harvard.edu/abs/2007MNRAS.380.1589B}
\bibitem[Baumgardt et al.(2010)]{Baumgardt2010}\linkup{autobib:Baumgardt2010} Baumgardt, H., Parmentier, G., Gieles, M., \& Vesperini, E.\ 2010, \mnras, 401, 1832\linkads{http://adsabs.harvard.edu/abs/2010MNRAS.401.1832B}
\bibitem[Bedin et al.(2004)]{Bedin2004}\linkup{autobib:Bedin2004} Bedin, L.~R., Piotto, G., Anderson, J., Cassisi, S., King, I.~R., Momany, Y., \& Carraro, G.\ 2004, \apjl, 605, L125\linkads{http://adsabs.harvard.edu/abs/2004ApJ...605L.125B}
\bibitem[Bekenstein \& Milgrom(1984)]{Bekenstein1984}\linkup{autobib:Bekenstein1984} Bekenstein, J., \& Milgrom, M.\ 1984, \apj, 286, 7\linkads{http://adsabs.harvard.edu/abs/1984ApJ...286....7B}
\bibitem[Bekki \& Mackey(2009)]{Bekki2009}\linkup{autobib:Bekki2009} Bekki, K., \& Mackey, A.~D.\ 2009, \mnras, 394, 124\linkads{http://adsabs.harvard.edu/abs/2009MNRAS.394..124B}
\bibitem[Binney \& Tremaine(1987)]{Binney1987}\linkup{autobib:Binney1987} Binney, J., \& Tremaine, S.\ 1987, Galactic Dynamics, First Edition, Princeton Univ. Press\linkads{http://adsabs.harvard.edu/abs/1987gady.book.....B}
\bibitem[Binney \& Tremaine(2008)]{Binney2008}\linkup{autobib:Binney2008} Binney, J., \& Tremaine, S.\ 2008, Galactic Dynamics, Second Edition, Princeton Univ. Press\linkads{http://adsabs.harvard.edu/abs/2008gady.book.....B}
\bibitem[Boily, Kroupa, \& Pe{\~n}arrubia-Garrido(2001)]{Boily2001}\linkup{autobib:Boily2001} Boily, C.~M., Kroupa, P., \& Pe{\~n}arrubia-Garrido, J.\ 2001, New Astronomy, 6, 27\linkads{http://adsabs.harvard.edu/abs/2001NewA....6...27B}
\bibitem[Boily \& Kroupa(2003a)]{Boily2003a}\linkup{autobib:Boily2003a} Boily, C.~M., \& Kroupa, P.\ 2003a, \mnras, 338, 665\linkads{http://adsabs.harvard.edu/abs/2003MNRAS.338..665B}
\bibitem[Boily \& Kroupa(2003b)]{Boily2003b}\linkup{autobib:Boily2003b} Boily, C.~M., \& Kroupa, P.\ 2003b, \mnras, 338, 673\linkads{http://adsabs.harvard.edu/abs/2003MNRAS.338..673B}
\bibitem[Boily \& Athanassoula(2006)]{Boily2006}\linkup{autobib:Boily2006} Boily, C.~M., \& Athanassoula, E.\ 2006, \mnras, 369, 608\linkads{http://adsabs.harvard.edu/abs/2006MNRAS.369..608B}
\bibitem[Bournaud, Jog, \& Combes(2005)]{Bournaud2005}\linkup{autobib:Bournaud2005} Bournaud, F., Jog, C.~J., \& Combes, F.\ 2005, \aap, 437, 69\linkads{http://adsabs.harvard.edu/abs/2005A\%26A...437...69B}
\bibitem[Boutloukos \& Lamers(2003)]{Boutloukos2003}\linkup{autobib:Boutloukos2003} Boutloukos, S.~G., \& Lamers, H.~J.~G.~L.~M.\ 2003, \mnras, 338, 717\linkads{http://adsabs.harvard.edu/abs/2003MNRAS.338..717B}
\bibitem[Boylan-Kolchin et al.(2009)]{Boylan2009}\linkup{autobib:Boylan2009} Boylan-Kolchin, M., Springel, V., White, S.~D.~M., Jenkins, A., \& Lemson, G.\ 2009, \mnras, 398, 1150\linkads{http://adsabs.harvard.edu/abs/2009MNRAS.398.1150B}
\bibitem[Brandl et al.(2005)]{Brandl2005}\linkup{autobib:Brandl2005} Brandl, B.~R., et al.\ 2005, \apj, 635, 280\linkads{http://adsabs.harvard.edu/abs/2005ApJ...635..280B}
\bibitem[Brodie \& Strader(2006)]{Brodie2006}\linkup{autobib:Brodie2006} Brodie, J.~P., \& Strader, J.\ 2006, \araa, 44, 193\linkads{http://adsabs.harvard.edu/abs/2006ARA\%26A..44..193B}
\bibitem[Bruzual \& Charlot(2003)]{Bruzual2003}\linkup{autobib:Bruzual2003} Bruzual, G., \& Charlot, S.\ 2003, \mnras, 344, 1000\linkads{http://adsabs.harvard.edu/abs/2003MNRAS.344.1000B}
\bibitem[Bushouse, Telesco, \& Werner(1998)]{Bushouse1998}\linkup{autobib:Bushouse1998} Bushouse, H.~A., Telesco, C.~M., \& Werner, M.~W.\ 1998, \aj, 115, 938\linkads{http://adsabs.harvard.edu/abs/1998AJ....115..938B}
\bibitem[Cappa \& Benaglia(1998)]{Cappa1998}\linkup{autobib:Cappa1998} Cappa, C.~E., \& Benaglia, P.\ 1998, \aj, 116, 1906\linkads{http://adsabs.harvard.edu/abs/1998AJ....116.1906C}
\bibitem[Cardone, Piedipalumbo, \& Tortora(2005)]{Cardone2005}\linkup{autobib:Cardone2005} Cardone, V.~F., Piedipalumbo, E., \& Tortora, C.\ 2005, \mnras, 358, 1325\linkads{http://adsabs.harvard.edu/abs/2005MNRAS.358.1325C}
\bibitem[Carr(1994)]{Carr1994}\linkup{autobib:Carr1994} Carr, B.\ 1994, \araa, 32, 531\linkads{http://adsabs.harvard.edu/abs/1994ARA\%26A..32..531C}
\bibitem[Castor, McCray, \& Weaver(1975)]{Castor1975}\linkup{autobib:Castor1975} Castor, J., McCray, R., \& Weaver, R.\ 1975, \apjl, 200, L107\linkads{http://adsabs.harvard.edu/abs/1975ApJ...200L.107C}
\bibitem[Chandar, Fall, \& Whitmore(2006)]{Chandar2006}\linkup{autobib:Chandar2006} Chandar, R., Fall, S.~M., \& Whitmore, B.~C.\ 2006, \apjl, 650, L111\linkads{http://adsabs.harvard.edu/abs/2006ApJ...650L.111C}
\bibitem[Chandrasekhar(1943)]{Chandrasekhar1943}\linkup{autobib:Chandrasekhar1943} Chandrasekhar, S.\ 1943, \apj, 97, 255\linkads{http://adsabs.harvard.edu/abs/1943ApJ....97..255C}
\bibitem[D'Ercole et al.(2008)]{DErcole2008}\linkup{autobib:DErcole2008} D'Ercole, A., Vesperini, E., D'Antona, F., McMillan, S.~L.~W., \& Recchi, S.\ 2008, \mnras, 391, 825\linkads{http://adsabs.harvard.edu/abs/2008MNRAS.391..825D}
\bibitem[Davis et al.(1985)]{Davis1985}\linkup{autobib:Davis1985} Davis, M., Efstathiou, G., Frenk, C.~S., \& White, S.~D.~M.\ 1985, \apj, 292, 371\linkads{http://adsabs.harvard.edu/abs/1985ApJ...292..371D}
\bibitem[de Blok(2010)]{deBlok2010}\linkup{autobib:deBlok2010} de Blok, W.~J.~G.\ 2010, Advances in Astronomy, 2010, 5\linkads{http://adsabs.harvard.edu/abs/2010AdAst2010....5D}
\bibitem[Decressin et al.(2007)]{Decressin2007}\linkup{autobib:Decressin2007} Decressin, T., Meynet, G., Charbonnel, C., Prantzos, N., \& Ekstr{\"o}m, S.\ 2007, \aap, 464, 1029\linkads{http://adsabs.harvard.edu/abs/2007A\%26A...464.1029D}
\bibitem[Decressin, Baumgardt, \& Kroupa(2008)]{Decressin2008}\linkup{autobib:Decressin2008} Decressin, T., Baumgardt, H., \& Kroupa, P.\ 2008, \aap, 492, 101\linkads{http://adsabs.harvard.edu/abs/2008A\%26A...492..101D}
\bibitem[Dehnen(1993)]{Dehnen1993}\linkup{autobib:Dehnen1993} Dehnen, W.\ 1993, \mnras, 265, 250\linkads{http://adsabs.harvard.edu/abs/1993MNRAS.265..250D}
\bibitem[Dehnen(2000)]{Dehnen2000}\linkup{autobib:Dehnen2000} Dehnen, W.\ 2000, \apjl, 536, L39\linkads{http://adsabs.harvard.edu/abs/2000ApJ...536L..39D}
\bibitem[Dehnen(2001)]{Dehnen2001}\linkup{autobib:Dehnen2001} Dehnen, W.\ 2001, \mnras, 324, 273\linkads{http://adsabs.harvard.edu/abs/2001MNRAS.324..273D}
\bibitem[Dekel, Devor, \& Hetzroni(2003)]{Dekel2003}\linkup{autobib:Dekel2003} Dekel, A., Devor, J., \& Hetzroni, G.\ 2003, \mnras, 341, 326\linkads{http://adsabs.harvard.edu/abs/2003MNRAS.341..326D}
\bibitem[di Matteo et al.(2007)]{diMatteo2007}\linkup{autobib:diMatteo2007} di Matteo, P., Combes, F., Melchior, A.-L., \& Semelin, B.\ 2007, \aap, 468, 61\linkads{http://adsabs.harvard.edu/abs/2007A\%26A...468...61d}
\bibitem[di Matteo et al.(2008)]{diMatteo2008}\linkup{autobib:diMatteo2008} di Matteo, P., Bournaud, F., Martig, M., Combes, F., Melchior, A.-L., \& Semelin, B.\ 2008, \aap, 492, 31\linkads{http://adsabs.harvard.edu/abs/2008A\%26A...492...31d}
\bibitem[Dieball, M{\"u}ller, \& Grebel(2002)]{Dieball2002}\linkup{autobib:Dieball2002} Dieball, A., M{\"u}ller, H., \& Grebel, E.~K.\ 2002, \aap, 391, 547\linkads{http://adsabs.harvard.edu/abs/2002A\%26A...391..547D}
\bibitem[Dobbs et al.(2010)]{Dobbs2010}\linkup{autobib:Dobbs2010} Dobbs, C.~L., Theis, C., Pringle, J.~E., \& Bate, M.~R.\ 2010, \mnras, 403, 625\linkads{http://adsabs.harvard.edu/abs/2010MNRAS.403..625D}
\bibitem[Draine \& Salpeter(1979)]{Draine1979}\linkup{autobib:Draine1979} Draine, B.~T., \& Salpeter, E.~E.\ 1979, \apj, 231, 438\linkads{http://adsabs.harvard.edu/abs/1979ApJ...231..438D}
\bibitem[Drake et al.(2007)]{Drake2007}\linkup{autobib:Drake2007} Drake, A.~J., Djorgovski, S.~G., Williams, R., Mahabal, A., Graham, M.~J., Christensen, E., Beshore, E.~C., \& Larson, S.~M.\ 2007, CBET, 1172, 1\linkads{http://adsabs.harvard.edu/abs/2007CBET.1172....1D}
\bibitem[Dubinski(2008)]{Dubinski2008}\linkup{autobib:Dubinski2008} Dubinski, J.\ 2008, New Journal of Physics, 10, 125002\linkads{http://adsabs.harvard.edu/abs/2008NJPh...10l5002D}
\bibitem[Duc \& Mirabel(1999)]{Duc1999}\linkup{autobib:Duc1999} Duc, P.-A., \& Mirabel, I.~F.\ 1999, Galaxy Interactions at Low and High Redshift, 186, 61\linkads{http://adsabs.harvard.edu/abs/1999IAUS..186...61D}
\bibitem[Duncan(1923)]{Duncan1923}\linkup{autobib:Duncan1923} Duncan, J.~C.\ 1923, \apj, 57, 137\linkads{http://adsabs.harvard.edu/abs/1923ApJ....57..137D}
\bibitem[Einasto(1965)]{Einasto1965}\linkup{autobib:Einasto1965} Einasto, J.\ 1965, Trudy Inst. Astroz. Alma-Ata, 51, 87
\bibitem[Elmegreen \& Efremov(1997)]{Elmegreen1997}\linkup{autobib:Elmegreen1997} Elmegreen, B.~G., \& Efremov, Y.~N.\ 1997, \apj, 480, 235\linkads{http://adsabs.harvard.edu/abs/1997ApJ...480..235E}
\bibitem[Elmegreen(2000)]{Elmegreen2000}\linkup{autobib:Elmegreen2000} Elmegreen, B.~G.\ 2000, \apj, 530, 277\linkads{http://adsabs.harvard.edu/abs/2000ApJ...530..277E}
\bibitem[Eneev, Kozlov, \& Sunyaev(1973)]{Eneev1973}\linkup{autobib:Eneev1973} Eneev, T.~M., Kozlov, N.~N., \& Sunyaev, R.~A.\ 1973, \aap, 22, 41\linkads{http://adsabs.harvard.edu/abs/1973A&A....22...41E}
\bibitem[Evans(1993)]{Evans1993}\linkup{autobib:Evans1993} Evans, N.~W.\ 1993, \mnras, 260, 191\linkads{http://adsabs.harvard.edu/abs/1993MNRAS.260..191E}
\bibitem[Fabbiano, Zezas, \& Murray(2001)]{Fabbiano2001}\linkup{autobib:Fabbiano2001} Fabbiano, G., Zezas, A., \& Murray, S.~S.\ 2001, \apj, 554, 1035\linkads{http://adsabs.harvard.edu/abs/2001ApJ...554.1035F}
\bibitem[Fall \& Rees(1977)]{Fall1977}\linkup{autobib:Fall1977} Fall, S.~M., \& Rees, M.~J.\ 1977, \mnras, 181, 37P\linkads{http://adsabs.harvard.edu/abs/1977MNRAS.181...37F}
\bibitem[Fall \& Zhang(2001)]{Fall2001}\linkup{autobib:Fall2001} Fall, S.~M., \& Zhang, Q.\ 2001, \apj, 561, 751\linkads{http://adsabs.harvard.edu/abs/2001ApJ...561..751F}
\bibitem[Fall, Chandar, \& Whitmore(2005)]{Fall2005}\linkup{autobib:Fall2005} Fall, S.~M., Chandar, R., \& Whitmore, B.~C.\ 2005, \apjl, 631, L133\linkads{http://adsabs.harvard.edu/abs/2005ApJ...631L.133F}
\bibitem[Fleck et al.(2006)]{Fleck2006}\linkup{autobib:Fleck2006} Fleck, J.-J., Boily, C.~M., Lan{\c c}on, A., \& Deiters, S.\ 2006, \mnras, 369, 1392\linkads{http://adsabs.harvard.edu/abs/2006MNRAS.369.1392F}
\bibitem[Fleck(2007)]{Fleck2007}\linkup{autobib:Fleck2007} Fleck, J.-J.\ 2007, unpublished thesis\linkads[http://tel.archives-ouvertes.fr/tel-00184822]{http://tel.archives-ouvertes.fr/tel-00184822}
\bibitem[Fortin(2006)]{Fortin2006}\linkup{autobib:Fortin2006} Fortin, P.\ 2006, unpublished thesis\linkads[http://tel.archives-ouvertes.fr/tel-00135843]{http://tel.archives-ouvertes.fr/tel-00135843}
\bibitem[Freeman(1970)]{Freeman1970}\linkup{autobib:Freeman1970} Freeman, K.~C.\ 1970, \apj, 160, 811\linkads{http://adsabs.harvard.edu/abs/1970ApJ...160..811F}
\bibitem[Geyer \& Burkert(2001)]{Geyer2001}\linkup{autobib:Geyer2001} Geyer, M.~P., \& Burkert, A.\ 2001, \mnras, 323, 988\linkads{http://adsabs.harvard.edu/abs/2001MNRAS.323..988G}
\bibitem[Gieles, Athanassoula, \& Portegies Zwart(2007)]{Gieles2007a}\linkup{autobib:Gieles2007a} Gieles, M., Athanassoula, E., \& Portegies Zwart, S.~F.\ 2007, \mnras, 376, 809\linkads{http://adsabs.harvard.edu/abs/2007MNRAS.376..809G}
\bibitem[Gieles, Lamers, \& Portegies Zwart(2007)]{Gieles2007b}\linkup{autobib:Gieles2007b} Gieles, M., Lamers, H.~J.~G.~L.~M., \& Portegies Zwart, S.~F.\ 2007, \apj, 668, 268\linkads{http://adsabs.harvard.edu/abs/2007ApJ...668..268G}
\bibitem[Gieles \& Baumgardt(2008)]{Gieles2008}\linkup{autobib:Gieles2008} Gieles, M., \& Baumgardt, H.\ 2008, \mnras, 389, L28\linkads{http://adsabs.harvard.edu/abs/2008MNRAS.389L..28G}
\bibitem[Gieles(2009)]{Gieles2009}\linkup{autobib:Gieles2009} Gieles, M.\ 2009, \mnras, 394, 2113\linkads{http://adsabs.harvard.edu/abs/2009MNRAS.394.2113G}
\bibitem[Gieles, Sana, \& Portegies Zwart(2010)]{Gieles2010}\linkup{autobib:Gieles2010} Gieles, M., Sana, H., \& Portegies Zwart, S.~F.\ 2010, \mnras, 402, 1750\linkads{http://adsabs.harvard.edu/abs/2010MNRAS.402.1750G}
\bibitem[Gingold \& Monaghan(1977)]{Gingold1977}\linkup{autobib:Gingold1977} Gingold, R.~A., \& Monaghan, J.~J.\ 1977, \mnras, 181, 375\linkads{http://adsabs.harvard.edu/abs/1977MNRAS.181..375G}
\bibitem[Glatt et al.(2008)]{Glatt2008}\linkup{autobib:Glatt2008} Glatt, K., et al.\ 2008, \aj, 136, 1703\linkads{http://adsabs.harvard.edu/abs/2008AJ....136.1703G}
\bibitem[Gnedin, Hernquist, \& Ostriker(1999)]{Gnedin1999}\linkup{autobib:Gnedin1999} Gnedin, O.~Y., Hernquist, L., \& Ostriker, J.~P.\ 1999, \apj, 514, 109\linkads{http://adsabs.harvard.edu/abs/1999ApJ...514..109G}
\bibitem[Goodwin(1997)]{Goodwin1997}\linkup{autobib:Goodwin1997} Goodwin, S.~P.\ 1997, \mnras, 284, 785\linkads{http://adsabs.harvard.edu/abs/1997MNRAS.284..785G}
\bibitem[Guillard(2010)]{Guillard2010}\linkup{autobib:Guillard2010} Guillard, P.\ 2010, PhD thesis, Univ. Paris-Sud XI, arXiv:1001.3613\linkads{http://adsabs.harvard.edu/abs/2010arXiv1001.3613G}
\bibitem[Hansen \& Moore(2006)]{Hansen2006}\linkup{autobib:Hansen2006} Hansen, S.~H., \& Moore, B.\ 2006, New Astronomy, 11, 333\linkads{http://adsabs.harvard.edu/abs/2006NewA...11..333H}
\bibitem[Harris(1991)]{Harris1991}\linkup{autobib:Harris1991} Harris, W.~E.\ 1991, \araa, 29, 543\linkads{http://adsabs.harvard.edu/abs/1991ARA\%26A..29..543H}
\bibitem[Hayashi \& Navarro(2006)]{Hayashi2006}\linkup{autobib:Hayashi2006} Hayashi, E., \& Navarro, J.~F.\ 2006, \mnras, 373, 1117\linkads{http://adsabs.harvard.edu/abs/2006MNRAS.373.1117H}
\bibitem[Hayashi, Navarro, \& Springel(2007)]{Hayashi2007}\linkup{autobib:Hayashi2007} Hayashi, E., Navarro, J.~F., \& Springel, V.\ 2007, \mnras, 377, 50\linkads{http://adsabs.harvard.edu/abs/2007MNRAS.377...50H}
\bibitem[Healy et al.(2003)]{Healy2003}\linkup{autobib:Healy2003} Healy D., Rockmore D., Kostelec P. \& Moore S.\ 2003, Journal of Fourier Analysis and Applications, 9:4, 341
\bibitem[Heggie \& Mathieu(1986)]{Heggie1986}\linkup{autobib:Heggie1986} Heggie, D.~C., \& Mathieu, R.~D.\ 1986, The Use of Supercomputers in Stellar Dynamics, Eds. P.~Hut and S.~McMillan, 267, 233\linkads{http://adsabs.harvard.edu/abs/1986LNP...267..233H}
\bibitem[Hemsendorf, Sigurdsson, \& Spurzem(2002)]{Hemsendorf2002}\linkup{autobib:Hemsendorf2002} Hemsendorf, M., Sigurdsson, S., \& Spurzem, R.\ 2002, \apj, 581, 1256\linkads{http://adsabs.harvard.edu/abs/2002ApJ...581.1256H}
\bibitem[H{\'e}non(1961)]{Henon1961}\linkup{autobib:Henon1961} H{\'e}non, M.\ 1961, Annales d'Astrophysique, 24, 369\linkads{http://adsabs.harvard.edu/abs/1961AnAp...24..369H}
\bibitem[Hernquist(1990)]{Hernquist1990}\linkup{autobib:Hernquist1990} Hernquist, L.\ 1990, \apj, 356, 359\linkads{http://adsabs.harvard.edu/abs/1990ApJ...356..359H}
\bibitem[Hernquist(1993)]{Hernquist1993}\linkup{autobib:Hernquist1993} Hernquist, L.\ 1993, \apjs, 86, 389\linkads{http://adsabs.harvard.edu/abs/1993ApJS...86..389H}
\bibitem[Hibbard \& van Gorkom(1996)]{Hibbard1996}\linkup{autobib:Hibbard1996} Hibbard, J.~E., \& van Gorkom, J.~H.\ 1996, \aj, 111, 655\linkads{http://adsabs.harvard.edu/abs/1996AJ....111..655H}
\bibitem[Hibbard et al.(2001)]{Hibbard2001}\linkup{autobib:Hibbard2001} Hibbard, J.~E., van der Hulst, J.~M., Barnes, J.~E., \& Rich, R.~M.\ 2001, \aj, 122, 2969\linkads{http://adsabs.harvard.edu/abs/2001AJ....122.2969H}
\bibitem[Hibbard et al.(2005)]{Hibbard2005}\linkup{autobib:Hibbard2005} Hibbard, J.~E., et al.\ 2005, \apjl, 619, L87\linkads{http://adsabs.harvard.edu/abs/2005ApJ...619L..87H}
\bibitem[Hills(1980)]{Hills1980}\linkup{autobib:Hills1980} Hills, J.~G.\ 1980, \apj, 235, 986\linkads{http://adsabs.harvard.edu/abs/1980ApJ...235..986H}
\bibitem[Holmberg(1941)]{Holmberg1941}\linkup{autobib:Holmberg1941} Holmberg, E.\ 1941, \apj, 94, 385\linkads{http://adsabs.harvard.edu/abs/1941ApJ....94..385H}
\bibitem[Holtzman et al.(1992)]{Holtzman1992}\linkup{autobib:Holtzman1992} Holtzman, J.~A., et al.\ 1992, \aj, 103, 691\linkads{http://adsabs.harvard.edu/abs/1992AJ....103..691H}
\bibitem[Hubble(1929)]{Hubble1929}\linkup{autobib:Hubble1929} Hubble, E.~P.\ 1929, \apj, 69, 103\linkads{http://adsabs.harvard.edu/abs/1929ApJ....69..103H}
\bibitem[Hubble(1936)]{Hubble1936}\linkup{autobib:Hubble1936} Hubble, E.~P.\ 1936, Realm of the Nebulae, Oxford Univ. Press\linkads{http://adsabs.harvard.edu/abs/1936rene.book.....H}
\bibitem[Hummel \& van der Hulst(1986)]{Hummel1986}\linkup{autobib:Hummel1986} Hummel, E., \& van der Hulst, J.~M.\ 1986, \aap, 155, 151\linkads{http://adsabs.harvard.edu/abs/1986A\%26A...155..151H}
\bibitem[Hurley, Pols, \& Tout(2000)]{Hurley2000}\linkup{autobib:Hurley2000} Hurley, J.~R., Pols, O.~R., \& Tout, C.~A.\ 2000, \mnras, 315, 543\linkads{http://adsabs.harvard.edu/abs/2000MNRAS.315..543H}
\bibitem[Hwang et al.(2010)]{Hwang2010}\linkup{autobib:Hwang2010} Hwang, J.-S., Struck, C., Renaud, F., \& Appleton, P.~N.\ 2010, ASPC, 423, 232\linkads{http://adsabs.harvard.edu/abs/2010ASPC..423..232H}
\bibitem[Jaffe(1983)]{Jaffe1983}\linkup{autobib:Jaffe1983} Jaffe, W.\ 1983, \mnras, 202, 995\linkads{http://adsabs.harvard.edu/abs/1983MNRAS.202..995J}
\bibitem[Jeans(1915)]{Jeans1915}\linkup{autobib:Jeans1915} Jeans, J.~H.\ 1915, \mnras, 76, 70\linkads{http://adsabs.harvard.edu/abs/1915MNRAS..76...70J}
\bibitem[Jeon, Kim, \& Ann(2009)]{Jeon2009}\linkup{autobib:Jeon2009} Jeon, M., Kim, S.~S., \& Ann, H.~B.\ 2009, \apj, 696, 1899\linkads{http://adsabs.harvard.edu/abs/2009ApJ...696.1899J}
\bibitem[Johansson, Naab, \& Burkert(2009)]{Johansson2009}\linkup{autobib:Johansson2009} Johansson, P.~H., Naab, T., \& Burkert, A.\ 2009, \apj, 690, 802\linkads{http://adsabs.harvard.edu/abs/2009ApJ...690..802J}
\bibitem[Joseph \& Wright(1985)]{Joseph1985}\linkup{autobib:Joseph1985} Joseph, R.~D., \& Wright, G.~S.\ 1985, \mnras, 214, 87\linkads{http://adsabs.harvard.edu/abs/1985MNRAS.214...87J}
\bibitem[Kapferer et al.(2009)]{Kapferer2009}\linkup{autobib:Kapferer2009} Kapferer, W., Sluka, C., Schindler, S., Ferrari, C., \& Ziegler, B.\ 2009, \aap, 499, 87\linkads{http://adsabs.harvard.edu/abs/2009A\%26A...499...87K}
\bibitem[Karl et al.(2008)]{Karl2008}\linkup{autobib:Karl2008} Karl, S.~J., Naab, T., Johansson, P.~H., Theis, C., \& Boily, C.~M.\ 2008, Astronomische Nachrichten, 329, 1042\linkads{http://adsabs.harvard.edu/abs/2008AN....329.1042K}
\bibitem[Karl et al.(2010)]{Karl2010}\linkup{autobib:Karl2010} Karl, S.~J., Naab, T., Johansson, P.~H., Kotarba, H., Boily, C., Renaud, F., \& Theis, C.\ 2010, \apjl, 715, L88\linkads{http://adsabs.harvard.edu/abs/2010ApJ...715L..88K}
\bibitem[Katz(1992)]{Katz1992}\linkup{autobib:Katz1992} Katz, N.\ 1992, \apj, 391, 502\linkads{http://adsabs.harvard.edu/abs/1992ApJ...391..502K}
\bibitem[Kawai \& Makino(1998)]{Kawai1998}\linkup{autobib:Kawai1998} Kawai, A., \& Makino, J.\ 1998, arXiv:9812431\linkads{http://adsabs.harvard.edu/abs/1998astro.ph.12431K}
\bibitem[Kennicutt(1998)]{Kennicutt1998}\linkup{autobib:Kennicutt1998} Kennicutt, R.~C., Jr.\ 1998, \apj, 498, 541\linkads{http://adsabs.harvard.edu/abs/1998ApJ...498..541K}
\bibitem[Kim, Wise, \& Abel(2009)]{Kim2009}\linkup{autobib:Kim2009} Kim, J.-h., Wise, J.~H., \& Abel, T.\ 2009, \apjl, 694, L123\linkads{http://adsabs.harvard.edu/abs/2009ApJ...694L.123K}
\bibitem[King(1962)]{King1962}\linkup{autobib:King1962} King, I.\ 1962, \aj, 67, 471\linkads{http://adsabs.harvard.edu/abs/1962AJ.....67..471K}
\bibitem[King(1966)]{King1966}\linkup{autobib:King1966} King, I.\ 1966, \aj, 71, 64\linkads{http://adsabs.harvard.edu/abs/1966AJ.....71...64K}
\bibitem[Klessen, Burkert, \& Bate(1998)]{Klessen1998}\linkup{autobib:Klessen1998} Klessen, R.~S., Burkert, A., \& Bate, M.~R.\ 1998, \apjl, 501, L205\linkads{http://adsabs.harvard.edu/abs/1998ApJ...501L.205K}
\bibitem[Klessen \& Burkert(2001)]{Klessen2001}\linkup{autobib:Klessen2001} Klessen, R.~S., \& Burkert, A.\ 2001, \apj, 549, 386\linkads{http://adsabs.harvard.edu/abs/2001ApJ...549..386K}
\bibitem[Kopp(2008)]{Kopp2008}\linkup{autobib:Kopp2008} Kopp, J.\ 2008, Int. J. Mod. Phys., C19, 523\linkads{http://adsabs.harvard.edu/abs/2008IJMPC..19..523K}
\bibitem[Kouwenhoven \& de Grijs(2008)]{Kouwenhoven2008}\linkup{autobib:Kouwenhoven2008} Kouwenhoven, M.~B.~N., \& de Grijs, R.\ 2008, \aap, 480, 103\linkads{http://adsabs.harvard.edu/abs/2008A\%26A...480..103K}
\bibitem[Kroupa(2001)]{Kroupa2001}\linkup{autobib:Kroupa2001} Kroupa, P.\ 2001, \mnras, 322, 231\linkads{http://adsabs.harvard.edu/abs/2001MNRAS.322..231K}
\bibitem[Kuijken \& Dubinski(1994)]{Kuijken1994}\linkup{autobib:Kuijken1994} Kuijken, K., \& Dubinski, J.\ 1994, \mnras, 269, 13\linkads{http://adsabs.harvard.edu/abs/1994MNRAS.269...13K}
\bibitem[Kuijken \& Dubinski(1995)]{Kuijken1995}\linkup{autobib:Kuijken1995} Kuijken, K., \& Dubinski, J.\ 1995, \mnras, 277, 1341\linkads{http://adsabs.harvard.edu/abs/1995MNRAS.277.1341K}
\bibitem[Kundic \& Ostriker(1995)]{Kundic1995}\linkup{autobib:Kundic1995} Kundic, T., \& Ostriker, J.~P.\ 1995, \apj, 438, 702\linkads{http://adsabs.harvard.edu/abs/1995ApJ...438..702K}
\bibitem[Lada \& Lada(2003)]{Lada2003}\linkup{autobib:Lada2003} Lada, C.~J., \& Lada, E.~A.\ 2003, \araa, 41, 57\linkads{http://adsabs.harvard.edu/abs/2003ARA\%26A..41...57L}
\bibitem[Laine et al.(2003)]{Laine2003}\linkup{autobib:Laine2003} Laine, S., van der Marel, R.~P., Rossa, J., Hibbard, J.~E., Mihos, J.~C., B{\"o}ker, T., \& Zabludoff, A.~I.\ 2003, \aj, 126, 2717\linkads{http://adsabs.harvard.edu/abs/2003AJ....126.2717L}
\bibitem[Lamers et al.(2005)]{Lamers2005}\linkup{autobib:Lamers2005} Lamers, H.~J.~G.~L.~M., Gieles, M., Bastian, N., Baumgardt, H., Kharchenko, N.~V., \& Portegies Zwart, S.\ 2005, \aap, 441, 117\linkads{http://adsabs.harvard.edu/abs/2005A\%26A...441..117L}
\bibitem[Larsen(2004)]{Larsen2004}\linkup{autobib:Larsen2004} Larsen, S.~S.\ 2004, \aap, 416, 53\linkads{http://adsabs.harvard.edu/abs/2004A\%26A...416...53L}
\bibitem[Larsen(2009)]{Larsen2009}\linkup{autobib:Larsen2009} Larsen, S.~S.\ 2009, \aap, 494, 539\linkads{http://adsabs.harvard.edu/abs/2009A\%26A...494..539L}
\bibitem[Lee et al.(1999)]{Lee1999}\linkup{autobib:Lee1999} Lee, Y.-W., Joo, J.-M., Sohn, Y.-J., Rey, S.-C., Lee, H.-C., \& Walker, A.~R.\ 1999, \nat, 402, 55\linkads{http://adsabs.harvard.edu/abs/1999Natur.402...55L}
\bibitem[Lindzen \& Chapman(1969)]{Lindzen1969}\linkup{autobib:Lindzen1969} Lindzen, R.~S., \& Chapman, S.\ 1969, Space Science Reviews, 10, 3\linkads{http://adsabs.harvard.edu/abs/1969SSRv...10....3L}
\bibitem[Mac Low \& Klessen(2004)]{MacLow2004}\linkup{autobib:MacLow2004} Mac Low, M.-M., \& Klessen, R.~S.\ 2004, Reviews of Modern Physics, 76, 125\linkads{http://adsabs.harvard.edu/abs/2004RvMP...76..125M}
\bibitem[Ma{\'{\i}}z-Apell{\'a}niz(2001)]{MaizApellaniz2001}\linkup{autobib:MaizApellaniz2001} Ma{\'{\i}}z-Apell{\'a}niz, J.\ 2001, \apj, 563, 151\linkads{http://adsabs.harvard.edu/abs/2001ApJ...563..151M}
\bibitem[Martin et al.(2005)]{Martin2005}\linkup{autobib:Martin2005} Martin, D.~C., et al.\ 2005, \apjl, 619, L1\linkads{http://adsabs.harvard.edu/abs/2005ApJ...619L...1M}
\bibitem[Mart{\'{\i}}n, Cappa, \& Benaglia(2008)]{Martin2008}\linkup{autobib:Martin2008} Mart{\'{\i}}n, M.~C., Cappa, C.~E., \& Benaglia, P.\ 2008, RevMexAA Conference Series, 33, 164\linkads{http://adsabs.harvard.edu/abs/2008RMxAC..33..164M}
\bibitem[McCrady, Gilbert, \& Graham(2003)]{McCrady2003}\linkup{autobib:McCrady2003} McCrady, N., Gilbert, A.~M., \& Graham, J.~R.\ 2003, \apj, 596, 240\linkads{http://adsabs.harvard.edu/abs/2003ApJ...596..240M}
\bibitem[McMillan \& Dehnen(2007)]{McMillan2007}\linkup{autobib:McMillan2007} McMillan, P.~J., \& Dehnen, W.\ 2007, \mnras, 378, 541\linkads{http://adsabs.harvard.edu/abs/2007MNRAS.378..541M}
\bibitem[Mengel et al.(2005)]{Mengel2005}\linkup{autobib:Mengel2005} Mengel, S., Lehnert, M.~D., Thatte, N., \& Genzel, R.\ 2005, \aap, 443, 41\linkads{http://adsabs.harvard.edu/abs/2005A\%26A...443...41M}
\bibitem[Merritt(1996)]{Merritt1996}\linkup{autobib:Merritt1996} Merritt, D.\ 1996, \aj, 111, 2462\linkads{http://adsabs.harvard.edu/abs/1996AJ....111.2462M}
\bibitem[Merritt \& Fridman(1996)]{Merritt1996}\linkup{autobib:Merritt1996} Merritt, D., \& Fridman, T.\ 1996, \apj, 460, 136\linkads{http://adsabs.harvard.edu/abs/1996ApJ...460..136M}
\bibitem[Merritt et al.(2005)]{Merritt2005}\linkup{autobib:Merritt2005} Merritt, D., Navarro, J.~F., Ludlow, A., \& Jenkins, A.\ 2005, \apjl, 624, L85\linkads{http://adsabs.harvard.edu/abs/2005ApJ...624L..85M}
\bibitem[Meurer(1995)]{Meurer1995}\linkup{autobib:Meurer1995} Meurer, G.~R.\ 1995, \nat, 375, 742\linkads{http://adsabs.harvard.edu/abs/1995Natur.375..742M}
\bibitem[Meylan \& Heggie(1997)]{Meylan1997}\linkup{autobib:Meylan1997} Meylan, G., \& Heggie, D.~C.\ 1997, \aapr, 8, 1\linkads{http://adsabs.harvard.edu/abs/1997A\%26ARv...8....1M}
\bibitem[Michie(1963)]{Michie1963}\linkup{autobib:Michie1963} Michie, R.~W.\ 1963, \mnras, 125, 127\linkads{http://adsabs.harvard.edu/abs/1963MNRAS.125..127M}
\bibitem[Mihos, Bothun, \& Richstone(1993)]{Mihos1993}\linkup{autobib:Mihos1993} Mihos, J.~C., Bothun, G.~D., \& Richstone, D.~O.\ 1993, \apj, 418, 82\linkads{http://adsabs.harvard.edu/abs/1993ApJ...418...82M}
\bibitem[Milgrom(1983)]{Milgrom1983}\linkup{autobib:Milgrom1983} Milgrom, M.\ 1983, \apj, 270, 365\linkads{http://adsabs.harvard.edu/abs/1983ApJ...270..365M}
\bibitem[Milone et al.(2008)]{Milone2008}\linkup{autobib:Milone2008} Milone, A.~P., et al.\ 2008, \apj, 673, 241\linkads{http://adsabs.harvard.edu/abs/2008ApJ...673..241M}
\bibitem[Milone et al.(2009a)]{Milone2009a}\linkup{autobib:Milone2009a} Milone, A.~P., Bedin, L.~R., Piotto, G., \& Anderson, J.\ 2009a, \aap, 497, 755\linkads{http://adsabs.harvard.edu/abs/2009A\%26A...497..755M}
\bibitem[Milone et al.(2009b)]{Milone2009b}\linkup{autobib:Milone2009b} Milone, A.~P., Stetson, P.~B., Piotto, G., Bedin, L.~R., Anderson, J., Cassisi, S., \& Salaris, M.\ 2009b, \aap, 503, 755\linkads{http://adsabs.harvard.edu/abs/2009A\%26A...503..755M}
\bibitem[Mirabel et al.(1992)]{Mirabel1992}\linkup{autobib:Mirabel1992} Mirabel, I.~F., Dottori, H., \& Lutz, D.\ 1992, \aap, 256, L19\linkads{http://adsabs.harvard.edu/abs/1992A\%26A...256L..19M}
\bibitem[Moore et al.(1999)]{Moore1999}\linkup{autobib:Moore1999} Moore, B., Quinn, T., Governato, F., Stadel, J., \& Lake, G.\ 1999, \mnras, 310, 1147\linkads{http://adsabs.harvard.edu/abs/1999MNRAS.310.1147M}
\bibitem[Naab \& Burkert(2003)]{Naab2003}\linkup{autobib:Naab2003} Naab, T., \& Burkert, A.\ 2003, \apj, 597, 893\linkads{http://adsabs.harvard.edu/abs/2003ApJ...597..893N}
\bibitem[Naab, Jesseit, \& Burkert(2006)]{Naab2006}\linkup{autobib:Naab2006} Naab, T., Jesseit, R., \& Burkert, A.\ 2006, \mnras, 372, 839\linkads{http://adsabs.harvard.edu/abs/2006MNRAS.372..839N}
\bibitem[Navarro \& White(1993)]{Navarro1993}\linkup{autobib:Navarro1993} Navarro, J.~F., \& White, S.~D.~M.\ 1993, \mnras, 265, 271\linkads{http://adsabs.harvard.edu/abs/1993MNRAS.265..271N}
\bibitem[Navarro, Frenk, \& White(1997)]{Navarro1997}\linkup{autobib:Navarro1997} Navarro, J.~F., Frenk, C.~S., \& White, S.~D.~M.\ 1997, \apj, 490, 493\linkads{http://adsabs.harvard.edu/abs/1997ApJ...490..493N}
\bibitem[Navarro et al.(2004)]{Navarro2004}\linkup{autobib:Navarro2004} Navarro, J.~F., et al.\ 2004, \mnras, 349, 1039\linkads{http://adsabs.harvard.edu/abs/2004MNRAS.349.1039N}
\bibitem[Navarro et al.(2010)]{Navarro2010}\linkup{autobib:Navarro2010} Navarro, J.~F., et al.\ 2010, \mnras, 402, 21\linkads{http://adsabs.harvard.edu/abs/2010MNRAS.402...21N}
\bibitem[O'Connell, Gallagher, \& Hunter(1994)]{OConnell1994}\linkup{autobib:OConnell1994} O'Connell, R.~W., Gallagher, J.~S., III, \& Hunter, D.~A.\ 1994, \apj, 433, 65\linkads{http://adsabs.harvard.edu/abs/1994ApJ...433...65O}
\bibitem[Ocvirk et al.(2006)]{Ocvirk2006}\linkup{autobib:Ocvirk2006} Ocvirk, P., Pichon, C., Lan{\c c}on, A., \& Thi{\'e}baut, E.\ 2006, \mnras, 365, 46\linkads{http://adsabs.harvard.edu/abs/2006MNRAS.365...46O}
\bibitem[Oort(1932)]{Oort1932}\linkup{autobib:Oort1932} Oort, J.~H.\ 1932, \bain, 6, 249\linkads{http://adsabs.harvard.edu/abs/1932BAN.....6..249O}
\bibitem[Ostriker, Spitzer, \& Chevalier(1972)]{Ostriker1972}\linkup{autobib:Ostriker1972} Ostriker, J.~P., Spitzer, L., Jr., \& Chevalier, R.~A.\ 1972, \apjl, 176, L51\linkads{http://adsabs.harvard.edu/abs/1972ApJ...176L..51O}
\bibitem[Peebles(1982)]{Peebles1982}\linkup{autobib:Peebles1982} Peebles, P.~J.~E.\ 1982, \apjl, 263, L1\linkads{http://adsabs.harvard.edu/abs/1982ApJ...263L...1P}
\bibitem[Pflamm-Altenburg \& Kroupa(2009)]{PflammAltenburg2009}\linkup{autobib:PflammAltenburg2009} Pflamm-Altenburg, J., \& Kroupa, P.\ 2009, \mnras, 397, 488\linkads{http://adsabs.harvard.edu/abs/2009MNRAS.397..488P}
\bibitem[Pfleiderer \& Siedentopf(1961)]{Pfleiderer1961}\linkup{autobib:Pfleiderer1961} Pfleiderer, J., \& Siedentopf, H.\ 1961, Zeitschrift f\"ur Astrophysik, 51, 201\linkads{http://adsabs.harvard.edu/abs/1961ZA.....51..201P}
\bibitem[Piotto et al.(2005)]{Piotto2005}\linkup{autobib:Piotto2005} Piotto, G., et al.\ 2005, \apj, 621, 77\linkads{http://adsabs.harvard.edu/abs/2005ApJ...621...77P}
\bibitem[Piotto et al.(2007)]{Piotto2007}\linkup{autobib:Piotto2007} Piotto, G., et al.\ 2007, \apjl, 661, L53\linkads{http://adsabs.harvard.edu/abs/2007ApJ...661L..53P}
\bibitem[Piotto(2009)]{Piotto2009}\linkup{autobib:Piotto2009} Piotto, G.\ 2009, arXiv:0902.1422\linkads{http://adsabs.harvard.edu/abs/2009arXiv0902.1422P}
\bibitem[Plummer(1911)]{Plummer1911}\linkup{autobib:Plummer1911} Plummer, H.~C.\ 1911, \mnras, 71, 460\linkads{http://adsabs.harvard.edu/abs/1911MNRAS..71..460P}
\bibitem[Raddick et al.(2007)]{Raddick2007}\linkup{autobib:Raddick2007} Raddick, J., et al.\ 2007, BAAS, 38, 892\linkads{http://adsabs.harvard.edu/abs/2007AAS...211.9403R}
\bibitem[Renaud et al.(2008)]{Renaud2008}\linkup{autobib:Renaud2008} Renaud, F., Boily, C.~M., Fleck, J.-J., Naab, T., \& Theis, C.\ 2008, \mnras, 391, L98\linkads{http://adsabs.harvard.edu/abs/2008MNRAS.391L..98R}
\bibitem[Renaud et al.(2009)]{Renaud2009}\linkup{autobib:Renaud2009} Renaud, F., Boily, C.~M., Naab, T., \& Theis, C.\ 2009, \apj, 706, 67\linkads{http://adsabs.harvard.edu/abs/2009ApJ...706...67R}
\bibitem[Renaud, Boily, \& Theis(2010)]{Renaud2010a}\linkup{autobib:Renaud2010a} Renaud, F., Boily, C.~M, \& Theis, C.\ 2010, \mnras\ submitted
\bibitem[Renaud, Appleton, \& Xu(2010)]{Renaud2010b}\linkup{autobib:Renaud2010b} Renaud, F., Appleton, P.~N, \& Xu, K.~C.\ 2010, \apj\ submitted
\bibitem[Rownd \& Young(1999)]{Rownd1999}\linkup{autobib:Rownd1999} Rownd, B.~K., \& Young, J.~S.\ 1999, \aj, 118, 670\linkads{http://adsabs.harvard.edu/abs/1999AJ....118..670R}
\bibitem[Rubin, Ford, \& D'Odorico(1970)]{Rubin1970}\linkup{autobib:Rubin1970} Rubin, V.~C., Ford, W.~K.~J., \& D'Odorico, S.\ 1970, \apj, 160, 801\linkads{http://adsabs.harvard.edu/abs/1970ApJ...160..801R}
\bibitem[Salpeter(1955)]{Salpeter1955}\linkup{autobib:Salpeter1955} Salpeter, E.~E.\ 1955, \apj, 121, 161\linkads{http://adsabs.harvard.edu/abs/1955ApJ...121..161S}
\bibitem[Sanders \& McGaugh(2002)]{Sanders2002}\linkup{autobib:Sanders2002} Sanders, R.~H., \& McGaugh, S.~S.\ 2002, \araa, 40, 263\linkads{http://adsabs.harvard.edu/abs/2002ARA\%26A..40..263S}
\bibitem[Sarajedini \& Mancone(2007)]{Sarajedini2007}\linkup{autobib:Sarajedini2007} Sarajedini, A., \& Mancone, C.~L.\ 2007, \aj, 134, 447\linkads{http://adsabs.harvard.edu/abs/2007AJ....134..447S}
\bibitem[Saviane, Hibbard, \& Rich(2004)]{Saviane2004}\linkup{autobib:Saviane2004} Saviane, I., Hibbard, J.~E., \& Rich, R.~M.\ 2004, \aj, 127, 660\linkads{http://adsabs.harvard.edu/abs/2004AJ....127..660S}
\bibitem[Saviane et al.(2008)]{Saviane2008}\linkup{autobib:Saviane2008} Saviane, I., Momany, Y., da Costa, G.~S., Rich, R.~M., \& Hibbard, J.~E.\ 2008, \apj, 678, 179\linkads{http://adsabs.harvard.edu/abs/2008ApJ...678..179S}
\bibitem[Scalo(1998)]{Scalo1998}\linkup{autobib:Scalo1998} Scalo, J.\ 1998, The Stellar Initial Mass Function, 142, 201\linkads{http://adsabs.harvard.edu/abs/1998ASPC..142..201S}
\bibitem[Schechter(1976)]{Schechter1976}\linkup{autobib:Schechter1976} Schechter, P.\ 1976, \apj, 203, 29\linkads{http://adsabs.harvard.edu/abs/1976ApJ...203...29S}
\bibitem[Schmidt(1959)]{Schmidt1959}\linkup{autobib:Schmidt1959} Schmidt, M.\ 1959, \apj, 129, 243\linkads{http://adsabs.harvard.edu/abs/1959ApJ...129..243S}
\bibitem[Schmidt(1975)]{Schmidt1975}\linkup{autobib:Schmidt1975} Schmidt, K.-H.\ 1975, \apss, 34, 23\linkads{http://adsabs.harvard.edu/abs/1975Ap\%26SS..34...23S}
\bibitem[Schweizer(1978)]{Schweizer1978}\linkup{autobib:Schweizer1978} Schweizer, F.\ 1978, Structure and Properties of Nearby Galaxies, 77, 279\linkads{http://adsabs.harvard.edu/abs/1978IAUS...77..279S}
\bibitem[Schweizer et al.(2008)]{Schweizer2008}\linkup{autobib:Schweizer2008} Schweizer, F., et al.\ 2008, \aj, 136, 1482\linkads{http://adsabs.harvard.edu/abs/2008AJ....136.1482S}
\bibitem[S\'ersic(1968)]{Sersic1968}\linkup{autobib:Sersic1968} S\'ersic, J.~L.\ 1968, Atlas de Galaxies Australes, Univ. Nac. C\'ordoba\linkads{http://adsabs.harvard.edu/abs/1968adga.book.....S}
\bibitem[Shu(1969)]{Shu1969}\linkup{autobib:Shu1969} Shu, F.~H.\ 1969, \apj, 158, 505\linkads{http://adsabs.harvard.edu/abs/1969ApJ...158..505S}
\bibitem[Shu, Adams, \& Lizano(1987)]{Shu1987}\linkup{autobib:Shu1987} Shu, F.~H., Adams, F.~C., \& Lizano, S.\ 1987, \araa, 25, 23\linkads{http://adsabs.harvard.edu/abs/1987ARA\%26A..25...23S}
\bibitem[Spitzer(1940)]{Spitzer1940}\linkup{autobib:Spitzer1940} Spitzer, L.~J.\ 1940, \mnras, 100, 396\linkads{http://adsabs.harvard.edu/abs/1940MNRAS.100..396S}
\bibitem[Spitzer(1958)]{Spitzer1958}\linkup{autobib:Spitzer1958} Spitzer, L.~J.\ 1958, \apj, 127, 17\linkads{http://adsabs.harvard.edu/abs/1958ApJ...127...17S}
\bibitem[Spitzer(1987)]{Spitzer1987}\linkup{autobib:Spitzer1987} Spitzer, L.\ 1987, Princeton Univ. Press\linkads{http://adsabs.harvard.edu/abs/1987degc.book.....S}
\bibitem[Springel(2000)]{Springel2000}\linkup{autobib:Springel2000} Springel, V.\ 2000, \mnras, 312, 859\linkads{http://adsabs.harvard.edu/abs/2000MNRAS.312..859S}
\bibitem[Springel \& Hernquist(2003)]{Springel2003}\linkup{autobib:Springel2003} Springel, V., \& Hernquist, L.\ 2003, \mnras, 339, 289\linkads{http://adsabs.harvard.edu/abs/2003MNRAS.339..289S}
\bibitem[Springel(2005)]{Springel2005}\linkup{autobib:Springel2005a} Springel, V.\ 2005, \mnras, 364, 1105\linkads{http://adsabs.harvard.edu/abs/2005MNRAS.364.1105S}
\bibitem[Springel et al.(2005)]{Springel2005}\linkup{autobib:Springel2005b} Springel, V., et al.\ 2005, \nat, 435, 629\linkads{http://adsabs.harvard.edu/abs/2005Natur.435..629S}
\bibitem[Spurzem, Baumgardt \& Ibold(2003)]{Spurzem2003}\linkup{autobib:Spurzem2003} Spurzem, R., Baumgardt, H. \& Ibold, N., 2003,\\\linkads[ftp://ftp.ari.uni-heidelberg.de/pub/staff/spurzem/nb6mpi]{ftp://ftp.ari.uni-heidelberg.de/pub/staff/spurzem/nb6mpi}
\bibitem[Stadel et al.(2009)]{Stadel2009}\linkup{autobib:Stadel2009} Stadel, J., Potter, D., Moore, B., Diemand, J., Madau, P., Zemp, M., Kuhlen, M., \& Quilis, V.\ 2009, \mnras, 398, L21\linkads{http://adsabs.harvard.edu/abs/2009MNRAS.398L..21S}
\bibitem[Stewart et al.(2008)]{Stewart2008}\linkup{autobib:Stewart2008} Stewart, K.~R., Bullock, J.~S., Wechsler, R.~H., Maller, A.~H., \& Zentner, A.~R.\ 2008, \apj, 683, 597\linkads{http://adsabs.harvard.edu/abs/2008ApJ...683..597S}
\bibitem[Stewart(2009)]{Stewart2009}\linkup{autobib:Stewart2009} Stewart, K.~R.\ 2009, ASPC, 419, 243\linkads{http://adsabs.harvard.edu/abs/2009ASPC..419..243S} 
\bibitem[Sutherland \& Dopita(1993)]{Sutherland1993}\linkup{autobib:Sutherland1993} Sutherland, R.~S., \& Dopita, M.~A.\ 1993, \apjs, 88, 253\linkads{http://adsabs.harvard.edu/abs/1993ApJS...88..253S}
\bibitem[Tegmark et al.(2004)]{Tegmark2004}\linkup{autobib:Tegmark2004} Tegmark, M., et al.\ 2004, \apj, 606, 702\linkads{http://adsabs.harvard.edu/abs/2004ApJ...606..702T}
\bibitem[Teuben(1995)]{Teuben1995}\linkup{autobib:Teuben1995} Teuben, P.\ 1995, Astronomical Data Analysis Software and Systems IV, 77, 398\linkads{http://adsabs.harvard.edu/abs/1995ASPC...77..398T}
\bibitem[Teyssier(2002)]{Teyssier2002}\linkup{autobib:Teyssier2002} Teyssier, R.\ 2002, \aap, 385, 337\linkads{http://adsabs.harvard.edu/abs/2002A\%26A...385..337T}
\bibitem[Theis \& Kohle(2001)]{Theis2001}\linkup{autobib:Theis2001} Theis, C., \& Kohle, S.\ 2001, \aap, 370, 365\linkads{http://adsabs.harvard.edu/abs/2001A\%26A...370..365T}
\bibitem[Tiret \& Combes(2007)]{Tiret2007}\linkup{autobib:Tiret2007} Tiret, O., \& Combes, F.\ 2007, arXiv:0712.1459\linkads{http://adsabs.harvard.edu/abs/2007arXiv0712.1459T}
\bibitem[Tonry et al.(2000)]{Tonry2000}\linkup{autobib:Tonry2000} Tonry, J.~L., Blakeslee, J.~P., Ajhar, E.~A., \& Dressler, A.\ 2000, \apj, 530, 625\linkads{http://adsabs.harvard.edu/abs/2000ApJ...530..625T}
\bibitem[Toomre \& Toomre(1972)]{Toomre1972}\linkup{autobib:Toomre1972} Toomre, A., \& Toomre, J.\ 1972, \apj, 178, 623\linkads{http://adsabs.harvard.edu/abs/1972ApJ...178..623T}
\bibitem[Toomre(1977)]{Toomre1977}\linkup{autobib:Toomre1977} Toomre, A.\ 1977, Evolution of Galaxies and Stellar Populations, Yale Univ. Obs, New Haven, 401\linkads{http://adsabs.harvard.edu/abs/1977egsp.conf..401T}
\bibitem[Tremaine et al.(1994)]{Tremaine1994}\linkup{autobib:Tremaine1994} Tremaine, S., Richstone, D.~O., Byun, Y.-I., Dressler, A., Faber, S.~M., Grillmair, C., Kormendy, J., \& Lauer, T.~R.\ 1994, \aj, 107, 634\linkads{http://adsabs.harvard.edu/abs/1994AJ....107..634T}
\bibitem[Trimble(1987)]{Trimble1987}\linkup{autobib:Trimble1987} Trimble, V.\ 1987, \araa, 25, 425\linkads{http://adsabs.harvard.edu/abs/1987ARA\%26A..25..425T}
\bibitem[Valluri(1993)]{Valluri1993}\linkup{autobib:Valluri1993} Valluri, M.\ 1993, \apj, 408, 57\linkads{http://adsabs.harvard.edu/abs/1993ApJ...408...57V}
\bibitem[Verschueren(1990)]{Verschueren1990}\linkup{autobib:Verschueren1990} Verschueren, W.\ 1990, \aap, 234, 156\linkads{http://adsabs.harvard.edu/abs/1990A\%26A...234..156V}
\bibitem[Vesperini(1998)]{Vesperini1998}\linkup{autobib:Vesperini1998} Vesperini, E.\ 1998, \mnras, 299, 1019\linkads{http://adsabs.harvard.edu/abs/1998MNRAS.299.1019V}
\bibitem[von Hoerner(1960)]{vonHoerner1960}\linkup{autobib:vonHoerner1960} von Hoerner, S.\ 1960, Zeitschrift f\"ur Astrophysik, 50, 184\linkads{http://adsabs.harvard.edu/abs/1960ZA.....50..184V}
\bibitem[Wang et al.(2004)]{Wang2004}\linkup{autobib:Wang2004} Wang, Z., et al.\ 2004, \apjs, 154, 193\linkads{http://adsabs.harvard.edu/abs/2004ApJS..154..193W}
\bibitem[Watson et al.(1996)]{Watson1996}\linkup{autobib:Watson1996} Watson, A.~M., et al.\ 1996, \aj, 112, 534\linkads{http://adsabs.harvard.edu/abs/1996AJ....112..534W}
\bibitem[Weidner, Kroupa, \& Larsen(2004)]{Weidner2004}\linkup{autobib:Weidner2004} Weidner, C., Kroupa, P., \& Larsen, S.~S.\ 2004, \mnras, 350, 1503\linkads{http://adsabs.harvard.edu/abs/2004MNRAS.350.1503W}
\bibitem[White(1977)]{White1977}\linkup{autobib:White1977} White, S.~D.~M.\ 1977, \mnras, 179, 33\linkads{http://adsabs.harvard.edu/abs/1977MNRAS.179...33W}
\bibitem[Whitmore et al.(1993)]{Whitmore1993}\linkup{autobib:Whitmore1993} Whitmore, B.~C., Schweizer, F., Leitherer, C., Borne, K., \& Robert, C.\ 1993, \aj, 106, 1354\linkads{http://adsabs.harvard.edu/abs/1993AJ....106.1354W}
\bibitem[Whitmore \& Schweizer(1995)]{Whitmore1995}\linkup{autobib:Whitmore1995} Whitmore, B.~C., \& Schweizer, F.\ 1995, \aj, 109, 960\linkads{http://adsabs.harvard.edu/abs/1995AJ....109..960W}
\bibitem[Whitmore et al.(1999)]{Whitmore1999}\linkup{autobib:Whitmore1999} Whitmore, B.~C., Zhang, Q., Leitherer, C., Fall, S.~M., Schweizer, F., \& Miller, B.~W.\ 1999, \aj, 118, 1551\linkads{http://adsabs.harvard.edu/abs/1999AJ....118.1551W}
\bibitem[Whitmore, Chandar, \& Fall(2007)]{Whitmore2007}\linkup{autobib:Whitmore2007} Whitmore, B.~C., Chandar, R., \& Fall, S.~M.\ 2007, \aj, 133, 1067\linkads{http://adsabs.harvard.edu/abs/2007AJ....133.1067W}
\bibitem[Whitmore et al.(2010)]{Whitmore2010}\linkup{autobib:Whitmore2010} Whitmore, B.~C., et al.\ 2010, \aj, 140, 75\linkads{http://adsabs.harvard.edu/abs/2010AJ....140...75W}
\bibitem[Zezas \& Fabbiano(2002)]{Zezas2002}\linkup{autobib:Zezas2002} Zezas, A., \& Fabbiano, G.\ 2002, \apj, 577, 726\linkads{http://adsabs.harvard.edu/abs/2002ApJ...577..726Z}
\bibitem[Zhang \& Fall(1999)]{Zhang1999}\linkup{autobib:Zhang1999} Zhang, Q., \& Fall, S.~M.\ 1999, \apjl, 527, L81\linkads{http://adsabs.harvard.edu/abs/1999ApJ...527L..81Z}
\bibitem[Zwicky(1933)]{Zwicky1933}\linkup{autobib:Zwicky1933} Zwicky, F.\ 1933, Helvetica Physica Acta, 6, 110\linkads{http://adsabs.harvard.edu/abs/1933AcHPh...6..110Z}

